DISK: Differentiable Sparse Kernel Complex for Efficient Spatially-Variant Convolution

Image convolution with complex kernels is a fundamental operation in photography, scientific imaging, and animation effects, yet direct dense convolution is computationally prohibitive on resource-limited devices. Existing approximations, such as simulated annealing or low-rank decompositions, either lack efficiency or fail to capture non-convex kernels. We introduce a differentiable kernel decomposition framework that represents a target spatially-variant, dense, complex kernel using a set of sparse kernel samples. Our approach features (i) a decomposition that enables differentiable optimization of sparse kernels, (ii) a dedicated initialization strategy for non-convex shapes to avoid poor local minima, and (iii) a kernel-space interpolation scheme that extends single-kernel filtering to spatially varying filtering without retraining and additional runtime overhead. Experiments on Gaussian and non-convex kernels show that our method achieves higher fidelity than simulated annealing and significantly lower cost than low-rank decompositions. Our approach provides a practical solution for mobile imaging and real-time rendering, while remaining fully differentiable for integration into broader learning pipelines.

==> algos/rejection_sampling.tex <==
\begin{algorithm}[H]
\caption{Non-Convex Kernel Initialization via Rejection Sampling}
\label{alg:rejection-sampling}
\begin{algorithmic}[1]
\STATE \textbf{Input:} Target kernel $K$, Number of samples $N_s$
\STATE \textbf{Output:} Initial offsets for the first sparse kernel $O_0$
\STATE $M \gets \text{Coordinates of non-zero pixels in } K$
\STATE $S \gets |M|$
\STATE $r \gets \sqrt{S / (N_s \cdot \pi)}$ \COMMENT{Initial rejection radius}
\STATE $O_0 \gets \emptyset$ \COMMENT{Initialize empty set for offsets}

% \IF{$\text{each candidate coordinate } p \in M$}
\FOR{each candidate coordinate $p \in M$} 
    \IF{$|O_0| \ge N_s$} 
        \STATE \textbf{break}
    \ENDIF
    \IF{$\forall o \in O_0, \| p - o \| \ge r$}
        \STATE $O_0 \gets O_0 \cup \{p\}$ \COMMENT{Accept sample if it's not too close to others}
    \ENDIF
\ENDFOR

\IF{$|O_0| < N_s$}
    \STATE $N_{\text{rem}} \gets N_s - |O_0|$ \COMMENT{Handle case where not enough samples were found}
    \STATE $M_{\text{fill}} \gets \text{First } N_{\text{rem}} \text{ coordinates from a deterministic repetition of } M$
    \STATE $O_0 \gets O_0 \cup M_{\text{fill}}$
\ENDIF
\STATE $O_0 \gets O_0 - \text{center}(K)$ \COMMENT{Center the offsets}
\STATE \textbf{return} $O_0$
% \Return $O_0$
\end{algorithmic}
\end{algorithm}

==> figures/layer-abl-dove.tex <==
\begin{figure}[htb]
    \centering
    \begin{minipage}{0.38\columnwidth} % 调整宽度，确保两张图能并排显示
        \centering
        \includegraphics[width=\linewidth]{figures/layer_abl/plot_layer_abl_curve_dove.pdf}
    \end{minipage}
    \hfill 
    \begin{minipage}{0.3\columnwidth} % 调整宽度，确保两张图能并排显示
        \centering
        \vspace{-6pt}
        \includegraphics[width=\linewidth]{figures/layer_abl/layer_abl_dove.pdf}
    \end{minipage}
    \begin{minipage}{0.3\columnwidth} % 调整宽度，确保两张图能并排显示
        \centering
        \vspace{-6pt}
        \includegraphics[width=\linewidth]{figures/layer_abl/layer_abl_dove_temper.pdf}
    \end{minipage}
    \caption{Ablation results for various configurations of samples and layers on \emph{Dove} kernel.}
    \label{fig:layer-abl-dove}
\end{figure}

==> figures/sv-line.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{figures/plots/plot_sv-line-new-lpips.pdf}
    \caption{\textbf{Quantitative evaluation of spatially-varying kernel approximation.} We plot LPIPS error (Y-axis, log scale, lower is better) against a continuous kernel size parameter (X-axis) for eight different kernel shapes.}
    \label{fig:sv-lines}
\end{figure}

==> tables/tab-gaussian-ablation.tex <==
\begin{table}[htb]
\centering
\small % 调小一级字号
\setlength{\tabcolsep}{1.0pt} % 缩小列间距
\caption{Ablation results of filtering of Gaussian kernels on impulse response.}
\label{tab:ablation-gaussian}
% 1 (Variant) + 3 (gs5) + 3 (gs7) + 3 (gs9) + 3 (gs11) = 13 columns
\begin{tabular}{lcccccccccccc} % 'l' for the first column, 'c' for the rest
\toprule
\multirow{2}{*}{\diagbox{Variant}{Filter}} & \multicolumn{3}{c}{$\sigma=5$} & \multicolumn{3}{c}{$\sigma=7$} & \multicolumn{3}{c}{$\sigma=9$} & \multicolumn{3}{c}{$\sigma=11$} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
& PSNR$\uparrow$ & LPIPS$\downarrow$ & FLIP$\downarrow$ & PSNR$\uparrow$ & LPIPS$\downarrow$ & FLIP$\downarrow$ & PSNR$\uparrow$ & LPIPS$\downarrow$ & FLIP$\downarrow$ & PSNR$\uparrow$ & LPIPS$\downarrow$ & FLIP$\downarrow$ \\
\midrule
L1+KWS+IR  & 97.79 & \textbf{.0099} & \textbf{.2604} & \textbf{99.98} & \textbf{.0052} & \textbf{.4943} & \textbf{99.85} & \textbf{.0028} & \textbf{.1906} & \textbf{96.77} & \textbf{.0063} & \textbf{.3926} \\
L1+KWS+R    & 96.11 & .0150 & .5567 & 93.46 & .0181 & .6603 & 90.57 & .0256 & .4152 & 79.72 & .2737 & 2.670 \\
L1+IR           & \textbf{98.31} & .0117 & .3871 & 93.69 & .0394 & .7209 & 91.83 & .1142 & .9803 & 91.99 & .0942 & .7191 \\
L1+R        & 97.64 & .0191 & .4443 & 93.05 & .0705 & .7021 & 90.77 & .1606 & .9916 & 88.16 & .3198 & 1.226 \\
L2+KWS+IR  & 65.04 & 19.57 & 6.635 & 67.77 & 1.393 & 7.119 & 69.96 & .3123 & 7.156 & 71.80 & .1318 & 6.576 \\
L2+Inc       & 90.18 & .0849 & .8460 & 90.02 & .1433 & 1.066 & 83.84 & .2396 & 2.291 & 77.17 & .4472 & 4.389 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/tab-kernel-ablation.tex <==
\begin{table}[htb]
\centering
\small % 调小一级字号
\setlength{\tabcolsep}{2.5pt} % 缩小列间距
\caption{\textbf{Ablation on arbitrary kernels.} Our full model (SUM+SS+IR) achieves the best performance. SUM/SOFM: sum-to-one/softmax weight normalization. SS: sparse sampling initialization. IR/R: increasing/fixed-step radial initialization. Basic: random initialization. \chg{For LPIPS and FLIP scores, both lower is better.}}
\label{tab:ablation-arbitrary}
\begin{tabular}{lcccccccccccccccc} % 'l' for the first column, 'c' for the rest
\toprule
\multirow{2}{*}{\diagbox{Variant}{Filter}} & \multicolumn{2}{c}{\small Ampersand} & \multicolumn{2}{c}{Disk} & \multicolumn{2}{c}{Heart} & \multicolumn{2}{c}{Star4} & \multicolumn{2}{c}{Ring} & \multicolumn{2}{c}{4-Sided} & \multicolumn{2}{c}{6-Sided} & \multicolumn{2}{c}{Star} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13} \cmidrule(lr){14-15} \cmidrule(lr){16-17}
& \tiny LPIPS & \tiny FLIP & \tiny LPIPS & \tiny FLIP & \tiny LPIPS & \tiny FLIP & \tiny LPIPS & \tiny FLIP & \tiny LPIPS & \tiny FLIP & \tiny LPIPS & \tiny FLIP & \tiny LPIPS &  \tiny FLIP & \tiny LPIPS & \tiny FLIP \\
\midrule
SUM+SS+IR & \textbf{1.44} & 2.63 & \textbf{.240} & 3.53 & \textbf{.230} & 1.54 & .326 & \textbf{3.00} & \textbf{.426} & \textbf{2.46} & \textbf{.276} & \textbf{.375} & \textbf{.218} & \textbf{1.77} & .790 & \textbf{5.28} \\
SOFM+SS+IR & 2.39 & \textbf{2.61} & .242 & 3.54 & .248 & 1.58 & \textbf{.311} & 3.07 & .432 & 2.72 & .299 & .420 & .246 & 2.04 & .798 & 5.38 \\
SUM+SS+R & 1.94 & 3.12 & .251 & \textbf{3.48} & .236 & 1.50 & .386 & 3.48 & .441 & 2.60 & .285 & .492 & .336 & 2.10 & \textbf{.748} & 5.60 \\
SOFM+SS+R & 1.90 & 2.97 & .269 & 3.81 & .241 & \textbf{1.41} & .466 & 3.38 & .434 & 2.48 & .332 & .481 & .374 & 2.67 & .937 & 5.93 \\
SUM+R & 9.74 & 11.7 & .774 & 14.6 & 1.13 & 8.78 & 1.52 & 8.88 & 2.57 & 25.0 & 1.65 & 5.06 & .960 & 10.4 & 6.44 & 11.1 \\
SOFM+R & 9.70 & 11.7 & .773 & 14.6 & 1.13 & 8.78 & 1.52 & 8.88 & 2.57 & 25.0 & 1.65 & 5.06 & .961 & 10.4 & 6.44 & 11.0 \\
SS & 10.4 & 10.3 & .524 & 22.6 & .906 & 11.2 & 2.16 & 15.1 & 2.28 & 10.3 & 1.20 & 12.8 & .744 & 12.6 & 4.62 & 7.61 \\
Basic & 21.1 & 25.3 & 12.0 & 32.8 & 13.9 & 26.7 & 23.2 & 17.3 & 233 & 38.4 & 11.3 & 23.1 & 9.83 & 29.1 & 13.8 & 18.8 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/tab-memory.tex <==
\begin{table*}[h]
\centering
\small 
\setlength{\tabcolsep}{2.2pt} 
\caption{\textbf{Memory bandwidth and runtime comparison.} \chg{RB and WB denote read and write bandwidth (MB/frame), while RR and WR represent the \emph{relative increase} in bandwidth with respect to the \emph{Identical} (point sampling) baseline, rather than the raw ratio. Time indicates per-frame runtime (ms). The superscript $^{\star}$ marks 1D spatially varying (SV) kernels. $S\times P$ implies $S$ samples across $P$ passes.}}
\label{tab:memory}
\begin{tabular}{l *{12}{c}}
\toprule
& $\text{Identical}$ & $\text{GT}^{\star}$ & $24\times4^{\star}$ & $32\times4^{\star}$ & $49\times4^{\star}$ & $\text{GT}$ & $12\times4$ & $24\times4$ & $32\times4$ & $49\times2$ & $49\times4$ & $49\times6$ \\
\midrule
$\text{RB}$   & 31.68 & 67.75 & 53.47 & 52.92 & 49.99 & 66.83 & 44.31 & 47.97 & 43.95 & 37.90 & 42.11 & 48.52 \\
$\text{WB}$   & 25.63 & 90.27 & 41.56 & 41.56 & 39.92 & 89.17 & 29.11 & 32.52 & 28.20 & 30.62 & 33.10 & 35.16 \\
$\text{RR}($\%$)$   & 0     & 113.8 & 68.78 & 67.05 & 57.80 & 110.9 & 72.88 & 87.16 & 71.48 & 47.87 & 64.30 & 89.31 \\ 
$\text{WR}($\%$)$   & 0     & 252.2 & 62.15 & 62.15 & 55.75 & 247.9 & 13.58 & 26.88 & 10.03 & 19.47 & 29.15 & 37.18 \\
$\text{Time}$ & 1.04  & 192.4 & 12.66 & 16.78 & 23.29 & 246.8 & 6.13  & 7.50  & 8.36  & 7.72  & 9.11  & 12.56 \\
\bottomrule
\end{tabular}
\end{table*}

